Differentially Private Search Log Sanitization with Optimal Output Utility

Web search logs contain extremely sensitive data, as evidenced by the recent AOL incident. However, storing and analyzing search logs can be very useful for many purposes (i.e. investigating human behavior). Thus, an important research question is how to privately sanitize search logs. Several search log anonymization techniques have been proposed with concrete privacy models. However, in all of these solutions, the output utility of the techniques is only evaluated rather than being maximized in any fashion. Indeed, for effective search log anonymization, it is desirable to derive the optimal (maximum utility) output while meeting the privacy standard. In this paper, we propose utility-maximizing sanitization based on the rigorous privacy standard of differential privacy, in the context of search logs. Specifically, we utilize optimization models to maximize the output utility of the sanitization for different applications, while ensuring that the production process satisfies differential privacy. An added benefit is that our novel randomization strategy ensures that the schema of the output is identical to that of the input. A comprehensive evaluation on real search logs validates the approach and demonstrates its robustness and scalability.

==> concl.tex <==
In this paper, we have addressed the important practical problem of
retaining the maximum utility while the search log sanitization
satisfies differential privacy and generates outputs with the
identical schema as the original search log. As a necessary step, we
have defined three different notions of utility that are useful for
various applications.
%We derived a set of linear constraints that
%guarantee differential privacy for the sanitization. We then
%formulate three different utility-maximizing problems that each
%maximizes the specific desired utility function while meeting the
%differential privacy constraints. We solved the utility-maximizing
%problems with effective and efficient solvers (Simplex algorithm
%with linear relaxation for O-UMP and F-UMP; SPE heuristic and NEOS
%solvers for D-UMP), and validated them using real data sets.
We have implemented our approach and validated it on several real data
sets.

We can extend our work in several directions. First, additional
notions of utility can be considered and corresponding optimization
models created. We also need to explore ways of combining different
utility notions to create a single joint objective.
%can be created that compromises different notions of utility.
This would be akin to a multi-objective optimization.
%The new utility
%notion based sanitization remains robust if the differential privacy
%constraints are satisfied.
Second, corresponding to the utility-maximizing problem, one can
similarly define the privacy breach-minimizing problem which asks
for minimal privacy loss while satisfying a certain utility. Third,
since we have modeled the utility-maximizing problems in the
optimization framework, it should be possible to leverage the
significant work in the field of operations research to solve these
problems. We intend to explore these in the future.


==> related.tex <==
\subsection{Search Log Anonymization}

Following the AOL search log incident, there has been some work on
user privacy issues related to privately publishing search logs.
Adar \cite{EAdar07} proposes a secret sharing scheme where a query
must appear at least $t$ times before it can be decoded. It may
potentially remove too many harmless queries, thus reducing data
utility. Kumar et al. \cite{KumarNPT07} propose an approach that
tokenizes each query tuple and hashes the corresponding search log
identifiers. However, inversion cannot be done using just the token
frequencies. Also, serious leaks are possible even when the order of
tokens is hidden.

More recently, some anonymization models
\cite{KorolovaKMN09,HeN09,HongCikm09,LiuW10} have been developed for
search log release. He et al. \cite{HeN09}, Hong et al.
\cite{HongCikm09} and Liu et al. \cite{LiuW10} anonymized search
logs based on k-anonymity which is not as rigorous as differential
privacy \cite{corn09}. Korolova et al. \cite{KorolovaKMN09} first
applied the rigorous privacy notion -- differential privacy to
search log release by adding Laplacian noise. However, several
shortcomings can be discovered in this work. First, the released
result of this is the statistical information of queries and clicks
where all users' search queries and clicks are aggregated together
(without individual attribution). The data utility might be greatly
reduced since the association between query-url pairs has been
removed (the published data in G{\"o}tz et al. \cite{corn09} also
suffers this constraint). With the released data, we cannot develop
personalized query suggestion or recommendation for search engines,
and also, we cannot carry out human behavior research since the
output data do not include the information that any two queries
belong to the same user. Second, as addressed by G{\"o}tz et al.
\cite{corn09}, the relaxed differential privacy notion in
\cite{KorolovaKMN09} is not sufficiently strong. Third, the utility
in \cite{KorolovaKMN09} is merely evaluated but not shown to be
maximized. Adding Laplacian noise to the counts of selected queries
and urls is straightforward and we cannot directly model
optimization problems to maximize the output utility. Alternatively,
our paper is to seek the maximum output utility for a novel
differentially private search log sanitization mechanism which
generate outputs with the identical schema as the original search
log.

Furthermore, G{\"o}tz et al. \cite{corn09} analyzes algorithms of
publishing frequent keywords, queries and clicks in search logs and
conducts a comparison w.r.t. two relaxations of
$\epsilon$-differential privacy (\textit{relaxations are
indispensable in search log publishing}). Our work utilizes the
stronger relaxation of $\epsilon$-differential privacy --
probabilistic differential privacy. Since we explore the optimal
utility in our differentially private sanitization mechanism which
outputs search logs rather than the results of counting queries and
clicked urls over the search log, our work has a completely
different focus, compared with their work \cite{corn09}.


\vspace{-0.05in}

\subsection{Differential Privacy}

In the context of relational data anonymization, Dwork et
al.\cite{DworkKMMN06,DworkMNSTcc06} have proposed the rigorous
privacy definition of differential privacy: a randomized algorithm
is differentially private if for any pair of neighboring inputs, the
probability of generating the same output, is within a small
multiple of each other. This means that for any two datasets which
are close to one another, a differentially private algorithm will
behave approximately the same on both data sets. This notion
provides sufficient privacy protection for users regardless of the
prior knowledge possessed by the adversaries. This has been extended
to data release in various different contexts besides search logs
(i.e. contingency tables, graph data). Specifically, Xiao et al.
\cite{XiaoWG10} introduced a data publishing technique which ensures
$\epsilon$-differential privacy while providing accurate answers for
range-count queries. Hay et al. \cite{HayLMJ09} presented an
efficient algorithm for releasing a provably private estimate of the
degree distribution of a network where it also satisfies the
differential privacy. McSherry et al. \cite{McSherryKDD09} solved
the problem of producing recommendations from collective user
behavior while providing differential privacy for users. Our work
follows the same line of research.

\subsection{Tradeoff between Privacy and Utility}

For any data modification based anonymization technique, a tradeoff
between privacy and utility naturally holds. Li et al.
\cite{LiLKdd09} analyzed the fundamental characteristics of privacy
and utility, and proposed a tradeoff framework for discussing
privacy and utility. In microdata disclosure, Bayardo et al.
\cite{BayardoA05} and LeFevre et al. \cite{LeFevreDR06} raised the
optimal k-anonymity and the optimal multidimensional anonymization
problem respectively. Kifer et al. \cite{utilitysigmod06} presented
a way to gain additional utility from k-anonymous and l-diverse
tables. Recently, Ghosh et al. \cite{utility} introduced a utility
maximizing mechanism for releasing a statistical database. However,
there is little work on this topic in the context of differential
privacy guaranteed search log release. To our knowledge, we takes a
first step towards addressing this deficiency.

